Mining Fix Patterns for FindBugs Violations

In this paper, we first collect and track a large number of fixed and unfixed violations across revisions of software. The empirical analyses reveal that there are discrepancies in the distributions of violations that are detected and those that are fixed, in terms of occurrences, spread and categories, which can provide insights into prioritizing violations. To automatically identify patterns in violations and their fixes, we propose an approach that utilizes convolutional neural networks to learn features and clustering to regroup similar instances. We then evaluate the usefulness of the identified fix patterns by applying them to unfixed violations. The results show that developers will accept and merge a majority (69/116) of fixes generated from the inferred fix patterns. It is also noteworthy that the yielded patterns are applicable to four real bugs in the Defects4J major benchmark for software testing and automated repair.

==> background.tex <==
\section{Motivation}
\label{sec:background}


% Moved background paragraphs into related work.

%This section presents the backgrounds of Word2Vec and convolutional neural networks.




==> table/comparison2.tex <==
\begin{table}[tp]
    \centering
    \setlength\tabcolsep{2pt}
    \caption{Comparison of distributions of fixed violation types against all detected violation types. {\em Ratio\_1} represents the occurred ratio of a given violation type in the all detected violations. {\em Ratio\_2} represents the occurred ratio of a given fixed violation type in all fixed violations. {\em R2/R1} is used to measure the fluctuation ratio of a violation type from all fixed violations to detected violations.}
    \label{tab:comparisonVTvsFVT}
    \resizebox{1.00\columnwidth}{!}{
    \begin{threeparttable}
        \begin{tabular}{c|lccc}
        \toprule
id & Top-50 fixed types & \makecell[c]{Ratio\_2(\%)} & \makecell[c]{Ratio\_1(\%)} & R2/R1\\
\hline 
1 & \tiny{SIC\_INNER\_SHOULD\_BE\_STATIC\_ANON} & {\bf8.81} & {\bf3.15} & {\bf2.80}\\
2 & \tiny{DLS\_DEAD\_LOCAL\_STORE} & {\bf5.74} & {\bf3.64} & {\bf1.58}\\
3 & \tiny{DM\_CONVERT\_CASE} & {\bf4.04} & {\bf1.89} & {\bf2.14}\\
4 & \tiny{DM\_DEFAULT\_ENCODING} & 3.52 & 2.49 & 1.41\\
5 & \tiny{UWF\_FIELD\_NOT\_INITIALIZED\_IN\_CONSTRUCTOR} & {\bf3.49} & {\bf2.29} & {\bf1.53}\\
6 & \tiny{RCN\_REDUNDANT\_NULLCHECK\_OF\_NONNULL\_VALUE} & 3.24 & 5.15 & 0.63\\
7 & \tiny{NM\_METHOD\_NAMING\_CONVENTION} & 2.89 & 2.77 & \textbf{\color{green}1.04}\\
8 & \tiny{URF\_UNREAD\_FIELD} & {\bf2.88} & {\bf1.26} & {\bf2.29}\\
9 & \tiny{BC\_UNCONFIRMED\_CAST} & 2.65 & 4.24 & 0.63\\
10 & \tiny{REC\_CATCH\_EXCEPTION} & 2.42 & 2.43 & \textbf{\color{green}1.00}\\
11 & \tiny{BC\_UNCONFIRMED\_CAST\_OF\_RETURN\_VALUE} & 2.25 & 2.02 & \textbf{\color{green}1.12}\\
12 & \tiny{SE\_NO\_SERIALVERSIONID} & 2.19 & 8.19 & 0.27\\
13 & \tiny{UPM\_UNCALLED\_PRIVATE\_METHOD} & {\bf2.16} & {\bf1.03} & {\bf2.10}\\
14 & \textbf{\tiny{VA\_FORMAT\_STRING\_USES\_NEWLINE}} & \textbf{\color{red}1.72} & \textbf{\color{red}0.25} & \textbf{\color{red}6.90}\\
15 & \tiny{MS\_SHOULD\_BE\_FINAL} & 1.71 & 1.72 & \textbf{\color{green}0.99}\\
16 & \tiny{RV\_RETURN\_VALUE\_IGNORED\_BAD\_PRACTICE} & 1.67 & 0.78 & {\bf2.15}\\
17 & \tiny{ST\_WRITE\_TO\_STATIC\_FROM\_INSTANCE\_METHOD} & 1.57 & 1.82 & \textbf{\color{green}0.87}\\
18 & \tiny{EI\_EXPOSE\_REP2} & 1.50 & 3.14 & 0.48\\
19 & \tiny{URF\_UNREAD\_PUBLIC\_OR\_PROTECTED\_FIELD} & 1.49 & 1.26 & \textbf{\color{green}1.18}\\
20 & \tiny{WMI\_WRONG\_MAP\_ITERATOR} & {\bf1.47} & {\bf0.72} & {\bf2.04}\\
21 & \tiny{OBL\_UNSATISFIED\_OBLIGATION} & {\bf1.40} & {\bf0.52} & {\bf2.69}\\
22 & \tiny{EI\_EXPOSE\_REP} & 1.35 & 3.20 & 0.42\\
23 & \tiny{NP\_LOAD\_OF\_KNOWN\_NULL\_VALUE} & 1.14 & 1.40 & \textbf{\color{green}0.82}\\
24 & \tiny{DM\_NUMBER\_CTOR} & 1.04 & 1.10 & \textbf{\color{green}0.94}\\
25 & \tiny{SIC\_INNER\_SHOULD\_BE\_STATIC} & 1.00 & 0.83 & 1.22\\
26 & \tiny{SBSC\_USE\_STRINGBUFFER\_CONCATENATION} & {\bf0.97} & {\bf0.48} & {\bf2.03}\\
27 & \tiny{OS\_OPEN\_STREAM\_EXCEPTION\_PATH} & {\bf0.91} & {\bf0.49} & {\bf1.87}\\
28 & \textbf{\tiny{NP\_NONNULL\_RETURN\_VIOLATION}} & \textbf{\color{red}0.87} & \textbf{\color{red}0.04} & \textbf{\color{red}23.00}\\
29 & \tiny{SF\_SWITCH\_NO\_DEFAULT} & 0.86 & 1.81 & 0.48\\
30 & \textbf{\tiny{UWF\_UNWRITTEN\_FIELD}} & \textbf{\color{red}0.84} & \textbf{\color{red}0.18} & \textbf{\color{red}4.73}\\
31 & \tiny{DE\_MIGHT\_IGNORE} & 0.79 & 0.71 & \textbf{\color{green}1.11}\\
32 & \tiny{IS2\_INCONSISTENT\_SYNC} & 0.71 & 0.99 & 0.72\\
33 & \textbf{\tiny{DM\_BOXED\_PRIMITIVE\_FOR\_PARSING}} & {\bf0.71} & {\bf0.24} & {\bf2.90}\\
34 & \textbf{\tiny{RV\_RETURN\_VALUE\_IGNORED\_NO\_SIDE\_EFFECT}} & {\bf0.64} & {\bf0.27} & {\bf2.42}\\
35 & \textbf{\tiny{ODR\_OPEN\_DATABASE\_RESOURCE}} & {\bf0.64} & {\bf0.22} & {\bf2.86}\\
36 & \tiny{PZLA\_PREFER\_ZERO\_LENGTH\_ARRAYS} & 0.63 & 2.19 & 0.29\\
37 & \tiny{RI\_REDUNDANT\_INTERFACES} & 0.62 & 1.91 & 0.32\\
38 & \textbf{\tiny{NP\_NULL\_ON\_SOME\_PATH\_FROM\_RETURN\_VALUE}} & {\bf0.61} & {\bf0.31} & {\bf1.99}\\
39 & \tiny{UCF\_USELESS\_CONTROL\_FLOW} & 0.61 & 0.53 & \textbf{\color{green}1.15}\\
40 & \tiny{UC\_USELESS\_CONDITION} & 0.59 & 0.39 & 1.49\\
41 & \textbf{\tiny{NP\_NULL\_ON\_SOME\_PATH}} & {\bf0.59} & {\bf0.29} & {\bf2.07}\\
42 & \textbf{\tiny{UC\_USELESS\_OBJECT}} & \textbf{\color{red}0.58} & \textbf{\color{red}0.15} & \textbf{\color{red}3.96}\\
43 & \tiny{DM\_FP\_NUMBER\_CTOR} & 0.57 & 0.40 & 1.43\\
44 & \tiny{MS\_PKGPROTECT} & 0.55 & 1.14 & 0.48\\
45 & \makecell[l]{\textbf{\tiny{SQL\_PREPARED\_STATEMENT\_GENERATED}}\tiny{\bf\_FROM\_NONCONSTANT\_STRING}} & {\bf0.55} & {\bf0.27} & {\bf2.07}\\
46 & \textbf{\tiny{OBL\_UNSATISFIED\_OBLIGATION\_EXCEPTION\_EDGE}} & {\bf0.55} & {\bf0.28} & {\bf1.96}\\
47 & \tiny{ES\_COMPARING\_STRINGS\_WITH\_EQ} & 0.51 & 0.52 & \textbf{\color{green}1.00}\\
48 & \textbf{\tiny{OS\_OPEN\_STREAM}} & 0.51 & 0.36 & 1.40\\
49 & \textbf{\tiny{RCN\_REDUNDANT\_NULLCHECK\_WOULD\_HAVE\_BEEN\_A\_NPE}} & {\bf0.50} & {\bf0.24} & {\bf2.08}\\
50 & \tiny{NP\_PARAMETER\_MUST\_BE\_NONNULL\_BUT\_MARKED\_AS\_NULLABLE} & 0.50 & 0.87 & 0.57\\
        \bottomrule
        \end{tabular}
    \end{threeparttable}
    }
\end{table}

==> table/fixedPatterns.tex <==
\begin{table*}[ht]
    \centering
    % \tiny
    \setlength\tabcolsep{2pt}
    \caption{Common source code patterns of fixed violations.}
    \label{tab:fixedSourceCodePatterns}
    \begin{threeparttable}
        \begin{tabular}{l|l}
        \toprule
        Violation Type     &  Common Source Code Pattern(s) \\
        \hline
% SIC\_INNER\_SHOULD\_BE\_STATIC\_ANON  & \makecell[l]{new Type() \{ override some methods(...)\{...\}\}.}\\
% DLS\_DEAD\_LOCAL\_STORE  & v1 = exp1, variable assignment statement.\\
DM\_CONVERT\_CASE  & \circled{1} stringExp.toLowerCase(),  \circled{2} stringExp.toUpperCase().\\ 
\hline
% DM\_DEFAULT\_ENCODING  & \makecell[l]{\circled{1} new BufferedReader(new InputStreamReader(input)), \\2) new StreamWriter(output); 3) stringExp.getBytes(),\\ 4) new String(byteExp), 5) byteExp.toString().}\\
% UWF\_FIELD\_NOT\_INITIALIZED\_IN\_CONSTRUCTOR  & null. \\ 
RCN\_REDUNDANT\_NULLCHECK\_OF\_NONNULL\_VALUE  & \circled{1} if (exp == null ...) \{...\}, \circled{2} if (exp != null ...) \{...\}. \\
% \textbf{\color{blue}NM\_METHOD\_NAMING\_CONVENTION}  & null.\\% (method body) \\
% URF\_UNREAD\_FIELD  & \circled{1} this.v1 = v2, \circled{2} this.v1 = new T(), \circled{3} private Type v = exp.\\ %\textbf{only pattern 3 is consistent.} 
\hline
BC\_UNCONFIRMED\_CAST  & \circled{1} T1 v1 = (T1) v2/exp, \circled{2} v1 = (T1) v2/exp, \circled{3} ((T1) v2).exp.\\
% \hline
% REC\_CATCH\_EXCEPTION  & try\{...\} catch (Exception e) \{...\}, Exception is not any specific exception.\\
% BC\_UNCONFIRMED\_CAST\_OF\_RETURN\_VALUE  & \makecell[l]{\circled{1} T1 v1 = (T1) method\_invocation(),  \circled{2} v1 = (T1) method\_invocation(),\\ \circled{3} ((T1) method\_invocation()).exp.}\\ 
% SE\_NO\_SERIALVERSIONID  & null. \\ 
% UPM\_UNCALLED\_PRIVATE\_METHOD  & null.\\ %(method body) \\ 
% \textbf{\color{red}VA\_FORMAT\_STRING\_USES\_NEWLINE}  & "$\backslash$n", this new line symbol is in a StringLiteral of a format method.\\ 
\hline
MS\_SHOULD\_BE\_FINAL  & public/protected/private static T1 v1 = exp.\\ %e.g., public static int maxStringLength = 65535. 
\hline
RV\_RETURN\_VALUE\_IGNORED\_BAD\_PRACTICE  & \makecell[l]{\circled{1} File.delete(), \circled{2} File.mkdirs(), \circled{3} File.mkdir(), \circled{4} File.createNewFile(), \\\circled{5} other exp.method\_invoation() returns a Boolean value.}\\ 
\hline
% ST\_WRITE\_TO\_STATIC\_FROM\_INSTANCE\_METHOD  & 1) static\_v1 = instance\_exp1.method\_invocation(), 2) v1 = instance\_exp1.method\_invocation(), 3) v1 = exp1, other variable assignment statement.\\ 
% EI\_EXPOSE\_REP2  & 1) this.v1 = v2, 2) v1 = v2. \textbf{inconsistent.}\\
% URF\_UNREAD\_PUBLIC\_OR\_PROTECTED\_FIELD  & \circled{1} this.v1 = v2, \circled{2} public/protected (static) T1 v1 = exp; \circled{3} v1 = exp1.\\ %\textbf{only 2 is consistent.}
% WMI\_WRONG\_MAP\_ITERATOR  & MapVariable.get(keyExp).\\ 
% OBL\_UNSATISFIED\_OBLIGATION  & \makecell[l]{1) StreamType v = new StreamType(...), 2) streamVariable = new StreamType(new StreamType2(...)), 3) sqlStatementExp.executeMethod(). \\e.g., 1. FileOutputStream fos = new FileOutputStream(outFile); 2. ResultSet rs = sqlStmt.executeQuery().\textbf{not very consistent.}} \\
% EI\_EXPOSE\_REP  & 1) return v; 2) return this.v;\\
% NP\_LOAD\_OF\_KNOWN\_NULL\_VALUE  & null.\\ 
DM\_NUMBER\_CTOR  & \makecell[l]{\circled{1} new Long(...), \circled{2} new Integer(...), \circled{3} new Short(...), \\\circled{4} new Byte(...), \circled{5} new Char(...).}\\
\hline
% SIC\_INNER\_SHOULD\_BE\_STATIC  & 1) this.v1 = v2; 2) v1 = v2; 3) super(...) \textbf{inaccurate localization of violation instances}\\ 
SBSC\_USE\_STRINGBUFFER\_CONCATENATION  & \circled{1} stringVariable += stringExp, \circled{2} stringVariable = stringExp1 + stringExp2.\\ 
\hline
% OS\_OPEN\_STREAM\_EXCEPTION\_PATH  & 1) StreamType v = new StreamType(...), 2) streamVariable = new StreamType(...).\textbf{not very consistent.}\\ 
% \textbf{\color{red}NP\_NONNULL\_RETURN\_VIOLATION}  & return null. \textbf{Inconsistent.}\\ 
% SF\_SWITCH\_NO\_DEFAULT  & switch(exp) \{case1:...case2:...\}, without default statement.\\ 
% \hline
% \textbf{\color{green}UWF\_UNWRITTEN\_FIELD}  & null.\\ 
% DE\_MIGHT\_IGNORE  & try\{...\} catch (Exception e) \{...\}, Exception is not any specified exception.\\%\textbf{To be discussed.} 
% IS2\_INCONSISTENT\_SYNC  & 1) return v1, 2) if(v1 != null) \{ v1.method\_invocation(); v1 = null;\}, 3)sqlStmt = stringLiteral1 + stringExp + stringLiteral2.\textbf{not very consistent.}\\ 
DM\_BOXED\_PRIMITIVE\_FOR\_PARSING  & \circled{1} Integer.valueOf(str), \circled{2} Long.valueOf(str). \\ 
% \textbf{\color{green}RV\_RETURN\_VALUE\_IGNORED\_NO\_SIDE\_EFFECT}  & method\_invocation\_exp, Method invocation statement returns a value, but does not assign the value to any variable. (High false positives.) \\ 
% \textbf{\color{red}ODR\_OPEN\_DATABASE\_RESOURCE}  & \makecell[l]{1) conn.createStatement(), 2) conn.createStatement.execute(...), \\3) PreparedStatement st = conn.prepareStatement(), 4)DataBaseConnection conn = exp.getConnection(...).}\\ 
\hline
PZLA\_PREFER\_ZERO\_LENGTH\_ARRAYS  & T[] methodName(...) \{... return null;\}. \\
% RI\_REDUNDANT\_INTERFACES  & super(...). \textbf{not very consistent. Locate on the position of super classes.}\\ 
% \textbf{\color{green}NP\_NULL\_ON\_SOME\_PATH\_FROM\_RETURN\_VALUE}  & File file = filesArray[index]/filesList.get(index). \\
% UCF\_USELESS\_CONTROL\_FLOW  & if (conditional expression) \{empty statements.\}.\\ 
% UC\_USELESS\_CONDITION  & if (conditional expression) \{...\}.\\ 
% \textbf{\color{green}NP\_NULL\_ON\_SOME\_PATH}  & null.\\ 
% \textbf{\color{green}UC\_USELESS\_OBJECT}  & T1 v1 = new T1().\\ 
% DM\_FP\_NUMBER\_CTOR  & \circled{1} new Double(exp), \circled{2} new Float(exp).\\ 
% MS\_PKGPROTECT  & public static (final) T1 v1 = initializationExp.\\ 
% \textbf{\color{red}SQL\_PREPARED\_STATEMENT\_GENERATED\_FROM\_NONCONSTANT\_STRING}  & sqlExecutionStatement = StringLiteral1 + stringV1 + StringLiteral2 + stringV2.\\ 
% \textbf{\color{green}OBL\_UNSATISFIED\_OBLIGATION\_EXCEPTION\_EDGE}  & \makecell[l]{1) StreamType v = new StreamType(...), 2) streamVariable = new StreamType(new StreamType2(...)), 3) sqlStatementExp.executeMethod(). \\e.g., 1. FileOutputStream fos = new FileOutputStream(outFile); 2. ResultSet rs = sqlStmt.executeQuery(). \textbf{not very consistent.}} \\ 
\hline
ES\_COMPARING\_STRINGS\_WITH\_EQ  & \circled{1} stringExp1 == stringExp2, \circled{2} stringExp1 != stringExp2.\\ 
% \textbf{\color{green}OS\_OPEN\_STREAM}  & \makecell[l]{1) StreamType v = new StreamType(...), 2) streamVariable = new StreamType(new StreamType2(...)), 3) sqlStatementExp.executeMethod(). \\e.g., 1. FileOutputStream fos = new FileOutputStream(outFile); 2. ResultSet rs = sqlStmt.executeQuery(). \textbf{the 3rd one is inconsistent.}} \\
% \textbf{\color{green}RCN\_REDUNDANT\_NULLCHECK\_WOULD\_HAVE\_BEEN\_A\_NPE}  & null.\\ 
% \textbf{\color{blue}NP\_PARAMETER\_MUST\_BE\_NONNULL\_BUT\_MARKED\_AS\_NULLABLE} & 1) method\_invocation(...), 2) class\_instance\_creation(...). \textbf{(not very consistent.)}\\
        \bottomrule
        \end{tabular}
    \end{threeparttable}
\end{table*}

